Bayesian Computing with INLA: A Review

The key operation in Bayesian inference, is to compute high-dimensional integrals. An old approximate technique is the Laplace method or approximation, which dates back to Pierre- Simon Laplace (1774). This simple idea approximates the integrand with a second order Taylor expansion around the mode and computes the integral analytically. By developing a nested version of this classical idea, combined with modern numerical techniques for sparse matrices, we obtain the approach of Integrated Nested Laplace Approximations (INLA) to do approximate Bayesian inference for latent Gaussian models (LGMs). LGMs represent an important model-abstraction for Bayesian inference and include a large proportion of the statistical models used today. In this review, we will discuss the reasons for the success of the INLA-approach, the R-INLA package, why it is so accurate, why the approximations are very quick to compute and why LGMs make such a useful concept for Bayesian computing.

==> Makefile <==
TARGETS = report.pdf 
DEPS_DIR = .deps
LATEXMK = latexmk -recorder -use-make -deps \
	-e 'warn qq(In Makefile, turn off custom dependencies\n);' \
	-e '@cus_dep_list = ();' \
	-e 'show_cus_dep();'
all : $(TARGETS)

$(foreach file,$(TARGETS),$(eval -include $(DEPS_DIR)/$(file)P))

$(DEPS_DIR) :
	mkdir $@

%.pdf : %.tex
	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
	$(LATEXMK) -pdf -dvi- -ps- -deps-out=$(DEPS_DIR)/$@P $<

%.png : %.pdf
	convert $< $@ 

clean :; latexmk -CA

.PHONY: clean

